Z-STAR+: A Zero-shot Style Transfer Method via Adjusting Style Distribution

Style transfer presents a significant challenge, primarily centered on identifying an appropriate style representation. Conventional methods employ style loss, derived from second-order statistics or contrastive learning, to constrain style representation in the stylized result. However, these pre-defined style representations often limit stylistic expression, leading to artifacts. In contrast to existing approaches, we have discovered that latent features in vanilla diffusion models inherently contain natural style and content distributions. This allows for direct extraction of style information and seamless integration of generative priors into the content image without necessitating retraining. Our method adopts dual denoising paths to represent content and style references in latent space, subsequently guiding the content image denoising process with style latent codes. We introduce a Cross-attention Reweighting module that utilizes local content features to query style image information best suited to the input patch, thereby aligning the style distribution of the stylized results with that of the style image. Furthermore, we design a scaled adaptive instance normalization to mitigate inconsistencies in color distribution between style and stylized images on a global scale. Through theoretical analysis and extensive experimentation, we demonstrate the effectiveness and superiority of our diffusion-based \uline{z}ero-shot \uline{s}tyle \uline{t}ransfer via \uline{a}djusting style dist\uline{r}ibution, termed Z-STAR+.

==> Figs/fig_compare_test.tex <==
\begin{figure*}%[h]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\linewidth]{image/compare.pdf}
\vspace{-15pt}
\caption{Qualitative comparisons of style transfer results using different methods.}
\label{fig:compare}
\vspace{-3pt}
\end{figure*}


==> Figs/fig_content_leak.tex <==
\newcommand\biascomparisonfigurewidth{0.075}
\newcommand\biascomparisontextwidth{0.015}

\begin{figure*}
\centering
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/c1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours1-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/StyleFormer-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/iest-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta1-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow1-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc1-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mast-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams1-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/sanet-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/avatar-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain1-1.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 1}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/s1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours1-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/StyleFormer-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/iest-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta1-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow1-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc1-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mast-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams1-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/sanet-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/avatar-20.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp1-20.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain1-20.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 20}}
\end{minipage}

% \begin{minipage}{\biascomparisontextwidth\linewidth}
%     \centering
%     \rotatebox{90}{\figtext{Style}}
% \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/s5.png}
% \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours5-20.png}
% \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta5-20.png}
% \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow5-20.png}
% \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc5-20.png}
% \end{minipage}
% % \begin{minipage}{\biascomparisonfigurewidth\linewidth}
% %     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-20.png}
% % \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams5-20.png}
% \end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain5-20.png}
% \end{minipage}
% \begin{minipage}{\biascomparisontextwidth\linewidth}
%     \centering
%     \rotatebox{90}{\figtext{Round 20}}
% \end{minipage}
\vspace{1pt}

\hspace{0.07\linewidth}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{StyleFormer}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{IEST}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{ArtFlow}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{MAST}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{SANet}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{Avatar}
\end{minipage}
\begin{minipage}[t]{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\vspace{-7pt}
\caption{Visualization of the content leak issue. Top/bottom: results after running the same stylization process using a certain method after the \engordnumber{1} and the \engordnumber{20} round, respectively.}
\vspace{-5pt}
\label{fig:content_leak}
\end{figure*}


==> Figs/fig_content_leak_s.tex <==
\newcommand\biascomparisonfigurewidth{0.13}
\newcommand\biascomparisontextwidth{0.015}

\begin{figure*}
\centering
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/c2.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours2-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta2-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow2-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc2-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams2-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain2-1.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 1}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth,height=\linewidth]{image/figs_bias_comparison/s2.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours2-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta2-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow2-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc2-20.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp1-20.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams2-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain2-20.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 20}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/c3.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours3-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta3-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow3-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc3-1.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-1.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams3-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain3-1.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 1}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth,height=\linewidth]{image/figs_bias_comparison/s3.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours3-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta3-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow3-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc3-20.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-20.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams3-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain3-20.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 20}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/c4.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours4-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta4-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow4-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc4-1.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-1.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams4-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain4-1.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 1}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth,height=\linewidth]{image/figs_bias_comparison/s4.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours4-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta4-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow4-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc4-20.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-20.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams4-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain4-20.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 20}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/c5.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours5-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta5-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow5-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc5-1.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-1.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams5-1.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain5-1.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 1}}
\end{minipage}

\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/s5.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/ours5-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/atta5-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/artflow5-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/mcc5-20.png}
\end{minipage}
% \begin{minipage}{\biascomparisonfigurewidth\linewidth}
%     \includegraphics[width=\linewidth]{image/figs_bias_comparison/dfp5-20.png}
% \end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/aams5-20.png}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_bias_comparison/adain5-20.png}
\end{minipage}
\begin{minipage}{\biascomparisontextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Round 20}}
\end{minipage}

\hspace{0.13\linewidth}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{ArtFlow}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\biascomparisonfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}
%\includegraphics[width= 0.99 \linewidth]{image/content_leak.pdf}
\vspace{-5pt}
\caption{Visualizations of the content leak issue.}
\vspace{-5pt}
\label{fig:content_leak_s}
\end{figure*}


==> Figs/fig_diff.tex <==
\begin{figure}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
 \rotatebox{90}{\includegraphics[width= 0.77\linewidth]{images/diff_compare.pdf}}
\caption{
% Compared with close-domain diffusion-based style transfer method. The effectiveness of StyleDiff is constrained when confronted with images that deviate from the specific training domain. This limitation is evident in the perplexing outcomes depicted in the first two columns of the third row.
%Differentiating itself from diffusion-based style transfer methods tailored for specific domains, 
% This constraint becomes evident when scrutinizing the perplexing outcomes presented in the first two columns of the third row.
Visual comparisons with StyleDiff.
As presented in the \nth{1} and \nth{2} columns, StyleDiff demonstrates limitations in effectively handling images that deviate from the training domain. 
Nevertheless, our method exhibits consistent and satisfactory performance across all types of input images.
}
% \vspace{-4mm}
\label{fig:diff}
\vspace{-10pt}
\end{figure}

==> Figs/fig_inst.tex <==
\begin{figure}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{images/inst_compare.pdf}
\caption{Compared with open-domain diffuison-based style transfer methods. Inst damage the content structure Seriously. The style in the results of VCT deviate from the references. }
% \vspace{-4mm}
\label{fig:inst}
\vspace{-10pt}
\end{figure}

==> Figs/fig_limitation.tex <==
\begin{figure}[h]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{image/bad_case.pdf}
\caption{Limitation of our StyTr$^2$ framework.
}
\label{fig:bad_case}
\end{figure}

==> Figs/fig_pe_visualization.tex <==
% \begin{figure}%[t]
%     \setlength{\abovecaptionskip}{2mm}
%     \centering
%     \includegraphics[width=\linewidth]{image/stytr2_cape_visual.pdf}
%     \vspace{-12pt}
%     \caption{Normalized attention scores of different types of PE.}
%     \label{fig:stytr2_cape_visual}
% \end{figure}

\begin{figure}
    \setlength{\abovecaptionskip}{2mm}
    \centering
    \begin{minipage}{\linewidth}
        \includegraphics[width=0.24\linewidth]{image/figs_pe_visualization/Learnable_PE.png}
        \includegraphics[width=0.24\linewidth]{image/figs_pe_visualization/Sinusoidal_PE.png}
        \includegraphics[width=0.24\linewidth]{image/figs_pe_visualization/CAPE1.png}
        \includegraphics[width=0.24\linewidth]{image/figs_pe_visualization/CAPE2.png}
    \end{minipage}
    \vspace{-1pt}
    \begin{minipage}{0.24\linewidth}
        \centering
        \figtext{Learnable PE}
    \end{minipage}
    \begin{minipage}{0.24\linewidth}
        \centering
        \figtext{Sinusoidal PE}
    \end{minipage}
    \begin{minipage}{0.48\linewidth}
        \centering
        \figtext{CAPE}
    \end{minipage}

    \caption{Normalized attention scores of different types of PE.}
    \label{fig:stytr2_cape_visual}
\end{figure}


==> Figs/fig_style_gradient.tex <==
\begin{figure}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{images/diff_style_gradient.pdf}
\caption{An illustration of horizontal styling gradient created by our method.}
% \vspace{-4mm}
\label{fig:style_grad}
\vspace{-10pt}
\end{figure}

==> Figs/fig_sup1.tex <==
\begin{figure*}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{images/experiment1.pdf}
\caption{Compared with other style transfer methods. The content images are presented in the first column, the style images are presented in the second column, and the stylized results generated by different methods are presented in the rest. 
}
% \vspace{-2mm}
\label{fig:sup1}
%\vspace{-10pt}
\end{figure*}

==> Figs/fig_sup2.tex <==
\begin{figure*}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{images/experiment2.pdf}
\caption{Compared with other style transfer methods. The content images are presented in the first column, the style images are presented in the second column, and the stylized results generated by different methods are presented in the rest. 
}
% \vspace{-2mm}
\label{fig:sup2}
%\vspace{-10pt}
\end{figure*}

==> Figs/fig_sup3.tex <==
\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow7.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc7.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams7.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain7.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow8.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}


\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc8.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams8.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain8.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow9.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc9.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams9.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain9.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\vspace{-7pt}
\caption{Comparisons of style transfer results using different methods.
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}
%\vspace{-2mm}
\label{fig:sup3}
\end{figure*}


==> Figs/fig_sup4.tex <==
\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow10.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc10.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams10.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain10.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow11.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc11.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams11.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain11.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/c12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/ours12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/atta12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/artflow12.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Ours}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaAttN}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Artflow}
\end{minipage}

\includegraphics[width=\supfigurewidth\linewidth,height=\supfigurewidth\linewidth]{image/figs_sups/s12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/mcc12.png}
% \includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/dfp1.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/aams12.png}
\includegraphics[width=\supfigurewidth\linewidth]{image/figs_sups/adain12.png}

\vspace{\supfigurespace}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{MCC}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AAMS}
\end{minipage}
\begin{minipage}{\supfigurewidth\linewidth}
    \centering
    \figtext{AdaIN}
\end{minipage}

\vspace{-7pt}
\caption{Comparisons of style transfer results using different methods.
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}
%\vspace{-2mm}
\label{fig:sup4}
\end{figure*}

==> Figs/fig_supp_ItoS.tex <==
% \begin{figure}%[!ht]
% \setlength{\abovecaptionskip}{2mm}
% \centering
% \includegraphics[width= \linewidth]{image/ItoS2.pdf}
% \caption{Comparisons of CNN and Linear projection through several rounds of image stylization.
% }
% \label{fig:ItoS2}
% \end{figure}

\newcommand\Ttosfigurewidth{0.22}
\newcommand\Ttostextwidth{0.015}
% \newcommand\nTtostextwidth{0.007}

\begin{figure}%[b]
\setlength{\abovecaptionskip}{2mm}
\centering

\begin{minipage}{\Ttostextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Style}}
\end{minipage}
\hspace{0pt}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/s.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/l1.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/l2.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/l3.png}
\end{minipage}
\begin{minipage}{\Ttostextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Linear}}
\end{minipage}

\begin{minipage}{\Ttostextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{Content}}
\end{minipage}
\hspace{0pt}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/c.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/cnn1.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/cnn2.png}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \includegraphics[width=\linewidth]{image/figs_ItoS2/cnn3.png}
\end{minipage}
\begin{minipage}{\Ttostextwidth\linewidth}
    \centering
    \rotatebox{90}{\figtext{CNN}}
\end{minipage}

\begin{minipage}{\Ttosfigurewidth\linewidth}
    \centering
    \figtext{Input}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \centering
    \figtext{Round 1}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \centering
    \figtext{Round 2}
\end{minipage}
\begin{minipage}{\Ttosfigurewidth\linewidth}
    \centering
    \figtext{Round 3}
\end{minipage}
\caption{Comparisons of CNN based and our linear projection based layers through several rounds of image stylization.
}
\vspace{-2mm}
\label{fig:ItoS2}
\end{figure}

==> Figs/fig_supp_big.tex <==
\newcommand\bigfigurewidth{0.31}

\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/c1.png}
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/r1.png}
\includegraphics[width=\bigfigurewidth\linewidth,height=\bigfigurewidth\linewidth]{image/figs_bigs/s1.png}


\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/c2.png}
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/r2.png}
\includegraphics[width=\bigfigurewidth\linewidth,height=\bigfigurewidth\linewidth]{image/figs_bigs/s2.png}

\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/c3.png}
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/r3.png}
\includegraphics[width=\bigfigurewidth\linewidth,height=\bigfigurewidth\linewidth]{image/figs_bigs/s3.png}

\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/c4.png}
\includegraphics[width=\bigfigurewidth\linewidth]{image/figs_bigs/r4.png}
\includegraphics[width=\bigfigurewidth\linewidth,height=\bigfigurewidth\linewidth]{image/figs_bigs/s4.png}

\vspace{-2pt}
\begin{minipage}{\bigfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\bigfigurewidth\linewidth}
    \centering
    \figtext{Our results}
\end{minipage}
\begin{minipage}{\bigfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\vspace{-7pt}
\caption{More style transfer results in a large resolution of $768 \times 768$.
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}\label{fig:big}
\end{figure*}


==> Figs/fig_supp_noise.tex <==
\begin{figure*}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\textwidth]{image/noise}
\caption{Comparisons of model robustness with ArtFlow. We visualize the impact of adding a small perturbation $\Delta$ following a Gaussian distribution on the stylized images in the \engordnumber{4} and \engordnumber{7} columns.
}
\label{fig:noise}
\end{figure*}


==> Figs/fig_supp_progressive.tex <==
\newcommand\pecomparisonfigurewidth{0.24}

\begin{figure}%[b]
\setlength{\abovecaptionskip}{2mm}
\centering
%\includegraphics[width=\linewidth]{image/pure_position.pdf}
\includegraphics[width=\pecomparisonfigurewidth\linewidth,height=\pecomparisonfigurewidth\linewidth]{image/figs_progressive/c.PNG}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{image/figs_progressive/single.PNG}
\includegraphics[width=\pecomparisonfigurewidth\linewidth]{image/figs_progressive/m.PNG}
\includegraphics[width=\pecomparisonfigurewidth\linewidth,height=\pecomparisonfigurewidth\linewidth]{image/figs_progressive/s.PNG}
% \includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s9.png}

\vspace{-4pt}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{Single-layer}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{Multi-layer}
\end{minipage}
\begin{minipage}[t]{\pecomparisonfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\caption{Impact of progressive generation of transformer decoder.}
\label{fig:progressive}
\end{figure}


==> Figs/fig_supp_weights.tex <==
% \begin{figure}%[!h]
% \setlength{\abovecaptionskip}{0mm}
% \centering
% \includegraphics[width= \linewidth]{image/weight.pdf}
% \caption{Impact of style weight.
% }
% \label{fig:weight}
% \end{figure}

\newcommand\weightfigurewidth{0.24}

\begin{figure}%[b]
\setlength{\abovecaptionskip}{2mm}
\centering
%\includegraphics[width=\linewidth]{image/pure_position.pdf}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/c1.png}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/wl1.png}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/wh1.png}
\includegraphics[width=\weightfigurewidth\linewidth,height=\pecomparisonfigurewidth\linewidth]{image/figs_weight/s1.png}
% \includegraphics[width=\comparisonfigurewidth\linewidth,height=\comparisonfigurewidth\linewidth]{image/figs_comparisons/s9.png}

\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/c2.png}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/wl2.png}
\includegraphics[width=\weightfigurewidth\linewidth]{image/figs_weight/wh2.png}
\includegraphics[width=\weightfigurewidth\linewidth,height=\pecomparisonfigurewidth\linewidth]{image/figs_weight/s2.png}

\vspace{-4pt}
\begin{minipage}[t]{\weightfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}[t]{\weightfigurewidth\linewidth}
    \centering
    \figtext{$\lambda_{s} = 5$}
\end{minipage}
\begin{minipage}[t]{\weightfigurewidth\linewidth}
    \centering
    \figtext{$\lambda_{s} = 10$}
\end{minipage}
\begin{minipage}[t]{\weightfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\caption{Impact of style weight.}
\vspace{-2mm}
\label{fig:weight}
\end{figure}


==> Figs/fig_teaser.tex <==
%\begin{figure*}[t]
%\setlength{\abovecaptionskip}{2mm}
%\centering
%\includegraphics[width=\linewidth]{image/intermediate_layers.pdf}
%\caption{
%Comparisons of intermediate layers using the rightmost image as both the content and the style image in a reconstruction task.
% (a) Our method. We decode the features extracted in the first three layers of our transformer decoder.
% The reconstruction results maintain distinct structures with increasing detailed brushstrokes.
% Since transformer can obtain long-range dependencies, the results generated by each layer look visually promising.
% (b) The CNN-based method proposed by Gatys et al.~\cite{gatys:2016:image}. We reconstruct the input image from from layers $conv1\_1$, $ \{ conv1\_1, conv2\_1 \}$, $\{conv1\_1, conv2\_1, conv3\_1, conv4\_1\}$ of a pretrained VGG network.
%(a) Image reconstruction results from layers $conv1\_1$, $ \{ conv1\_1, conv2\_1 \}$, $\{conv1\_1, conv2\_1, conv3\_1, conv4\_1\}$ of a pretrained VGG network based on Gatys et al.~\cite{gatys:2016:image}.
%(b) Feature visualizations of three layers of the transformer decoder.
% We find that reconstruction results match the style of a given image on an increasing scale as the network deepens.
% Different layers of CNN-based model focus on different scale information, thus it cannot generate satisfactory result by every layer.
%}
%\label{fig:pipline}
%\end{figure*}


\begin{center}
    \centering
    \captionsetup{type=figure}
\includegraphics[width=0.8 \linewidth]{image/p1.pdf}
\caption{
Our stylization results. Our method can generate promising stylized effect with well-preserved content structures and fine details.
}
\label{fig:teaser}
\end{center}

==> Figs/fig_user_study.tex <==
\begin{table*}%[!h]
\small
% \setlength\tabcolsep{9.5pt}
\centering
\begin{floatrow}

\capbtabbox{
\begin{tabular}{m{1.1cm}<{\centering}|m{0.7cm}<{\centering}m{0.5cm}<{\centering}m{0.5cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
\toprule
&ArtFlow&MCC&DFP& AAMS& AdaIN \\
\midrule
% Num. & 783&820&827&809&734 \\
votes &25.7&25.5&22.6&18.2& 23.5\\
% Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
\bottomrule
\end{tabular}
}{
% \vspace{-2mm}
\caption{User study results. }
% \vspace{-2mm}
\label{tab:user}
    }
\capbtabbox{
\begin{tabular}{m{1.1cm}<{\centering}|m{0.7cm}<{\centering}m{0.5cm}<{\centering}m{0.5cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
\toprule
&ArtFlow&MCC&DFP& AAMS& AdaIN \\
\midrule
% Num. & 783&820&827&809&734 \\
votes &25.7&25.5&22.6&18.2& 23.5\\
% Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
\bottomrule
\end{tabular}
}{
% \vspace{-2mm}
\caption{User study results. }
% \vspace{-2mm}
\label{tab:user}
    }
\capbtabbox{
\begin{tabular}{m{1.1cm}<{\centering}|m{0.7cm}<{\centering}m{0.5cm}<{\centering}m{0.5cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
\toprule
&ArtFlow&MCC&DFP& AAMS& AdaIN \\
\midrule
% Num. & 783&820&827&809&734 \\
votes &25.7&25.5&22.6&18.2& 23.5\\
% Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
\bottomrule
\end{tabular}
}{
% \vspace{-2mm}
\caption{User study results. }
% \vspace{-2mm}
\label{tab:user}
    }
\end{floatrow}
\vspace{-4mm}
\end{table*}

==> Figs/fig_vis.tex <==
\newcommand\teaserfigurewidth{0.23}
\newcommand\teasertextvspace{-2pt}

\begin{figure}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
%\includegraphics[width=\linewidth]{image/intermediate_layers.pdf}
\begin{minipage}{\teaserfigurewidth\linewidth}
\centering
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/input.png}
\end{minipage}
\vspace{\teasertextvspace}
%\begin{minipage}[t]{\linewidth}
\centering
\smallfigtext{\emph{Woman with a Hat}, Henri Matisse, 1905.}
%\end{minipage}
\end{minipage}
% 1st
\begin{minipage}{\teaserfigurewidth\linewidth}
\centering
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/cnn1.png}
\end{minipage}
\vspace{\teasertextvspace}
\begin{minipage}{\linewidth}
\centering
    \smallfigtext{conv1\_1}
\end{minipage}

\vspace{7pt}
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/ours1.png}
\end{minipage}
\vspace{\teasertextvspace}
\begin{minipage}{\linewidth}
\centering
    \smallfigtext{layer\_1}
\end{minipage}
%
\end{minipage}
% 2nd
\begin{minipage}{\teaserfigurewidth\linewidth}
\centering
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/cnn2.png}
\end{minipage}
\vspace{\teasertextvspace}
\begin{minipage}{\linewidth}
\centering
    \smallfigtext{\{conv1\_1,conv2\_1\}}
\end{minipage}

\vspace{7pt}
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/ours2.png}
\end{minipage}
\vspace{\teasertextvspace}
\begin{minipage}{\linewidth}
\centering
    \smallfigtext{layer\_2}
\end{minipage}
%
\end{minipage}
% 3nd
\begin{minipage}{\teaserfigurewidth\linewidth}
\centering
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/cnn3.png}
\end{minipage}
\vspace{\teasertextvspace}
\begin{minipage}{\linewidth}
\centering
    \smallfigtext{\{conv1\_1,...,conv4\_1\}}
\end{minipage}

\vspace{7pt}
\begin{minipage}{\linewidth}
    \includegraphics[width=\linewidth]{image/figs_features/ours3.png}
\end{minipage}
\vspace{\teasertextvspace}
\begin{minipage}{\linewidth}
\centering
    \smallfigtext{layer\_3}
\end{minipage}
%
\end{minipage}
% text
\begin{minipage}{0.03\linewidth}
    \centering
    \figtext{(a)}

    \vspace{55pt}

    \figtext{(b)}
\end{minipage}
\caption{Comparisons of intermediate layers using the leftmost image as the input content and the style reference in a style transfer task.
% (a) Our method. We decode the features extracted in the first three layers of our transformer decoder.
% The reconstruction results maintain distinct structures with increasing detailed brushstrokes.
% Since transformer can obtain long-range dependencies, the results generated by each layer look visually promising.
% (b) The CNN-based method proposed by Gatys et al.~\cite{gatys:2016:image}. We reconstruct the input image from from layers $conv1\_1$, $ \{ conv1\_1, conv2\_1 \}$, $\{conv1\_1, conv2\_1, conv3\_1, conv4\_1\}$ of a pretrained VGG network.
(a) Feature visualizations of a pretrained VGG based on Gatys \etal~\cite{gatys:2016:image}.
(b) Feature visualizations of our transformer decoder.
% We find that reconstruction results match the style of a given image on an increasing scale as the network deepens.
% Different layers of CNN-based model focus on different scale information, thus it cannot generate satisfactory result by every layer.
}
\label{fig:cnnvis}
%\vspace{-14pt}
%\label{fig:pipline}
\end{figure}


==> Figs/fig_vit.tex <==
\newcommand\vitfigurewidth{0.32}

\begin{figure}%[t]
%\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width=\vitfigurewidth\linewidth]{image/figs_vits/c1.png}
\includegraphics[width=\vitfigurewidth\linewidth]{image/figs_vits/r1.png}
\includegraphics[width=\vitfigurewidth\linewidth,height=\vitfigurewidth\linewidth]{image/figs_vits/s1.png}

\includegraphics[width=\vitfigurewidth\linewidth]{image/figs_vits/c2.png}
\includegraphics[width=\vitfigurewidth\linewidth]{image/figs_vits/r2.png}
\includegraphics[width=\vitfigurewidth\linewidth,height=\vitfigurewidth\linewidth]{image/figs_vits/s2.png}

\vspace{-5pt}
\begin{minipage}{\vitfigurewidth\linewidth}
    \centering
    \figtext{Content}
\end{minipage}
\begin{minipage}{\vitfigurewidth\linewidth}
    \centering
    \figtext{VIT}
\end{minipage}
\begin{minipage}{\vitfigurewidth\linewidth}
    \centering
    \figtext{Style}
\end{minipage}
\vspace{-7pt}
\caption{Style transfer results using model trained by VIT-based loss. 
% The first column shows content images, the second column shows style images. The remaining columns are stylized results generated by different methods.
}
%\vspace{-2mm}
\label{fig:vit}
\end{figure}


==> Figs/teaset.tex <==
\begin{figure*}%[t]
\setlength{\abovecaptionskip}{2mm}
\centering
\includegraphics[width= \linewidth]{images/fig1.pdf}
\caption{Our style transfer results compared with state-of-the-art methods.}
\label{fig:position}
\vspace{-10pt}
\end{figure*}


==> Sections/sup.tex <==
%\appendix

%\section{Method}
% \section{Network Architecture}
% In this section, we show the detailed sketch diagram of our CNN-based decoder and the self-supervised learning task.
% (a) The decoder uses three layers of $3 \times 3 \  \convolution + \relu + 2 \times \upsampling $ operators to increase the output resolution.
% (b) The self-supervised learning task uses the information of the input image. As shown in Fig.~\ref{fig:net2}, we input two same content (style) images into our $StyTr^2$, the generated image should be identical to the input content (style) image.

% \begin{figure*}%[h]
% \setlength{\abovecaptionskip}{2mm}
% \centering
% \includegraphics[width= \textwidth]{image/net2.pdf}
% \caption{Network architecture. (a) The three layers CNN-based decoder used to increase image resolution. (2) The self-supervised learning task used as a training aid.
% }
% \label{fig:net2}
% \end{figure*}

% \section{More Experimental Results}

% \subsection{Variance of Quantitative Evaluation}
% The quantitative evaluation is conducted by randomly selecting several content and style images.
% Therefore, we calculate the variance of content and style loss to show the random level.
% The statistics are shown in Table~\ref{tab:variance}. The content and style loss of StyTr$2$ is lower than others with a small value float.
% \begin{table*}[!h]
% \small
% \setlength\tabcolsep{2.5pt}
% \centering
% \begin{tabular}{c|cccccc}
% \toprule
%  &Ours&ArtFlow&MCC&DFP& AAMS& AdaIN \\
% \midrule

% $\mathcal{L}_c$   & \textbf{1.91 $\pm$ 0.114}&2.13 $\pm$ 0.207&2.38 $\pm$ 0.133 &2.67 $\pm$ 0.067 & 2.44 $\pm$ 0.097 & 2.34 $\pm$ 0.105\\
% $\mathcal{L}_s$     & \textbf{1.47 $\pm$ 0.950}&3.08 $\pm$ 1.800 &1.56$\pm$ 0.972 &2.12 $\pm$ 1.652 & 3.18 $\pm$ 2.070 & 1.91 $\pm$ 1.760\\
% % Var.($L_c$) & 0.114&0.207&0.133&0.067&0.097& 0.105 \\
% % Var.($L_s$) & 0.950&1.800&0.972& 1.650& 2.070& 1.760 \\

% \bottomrule
% \end{tabular}
% \caption{Variance of quantitative comparisons.}
% \label{tab:variance}
% \end{table*}

\section{Ablation Study}

%\paragraph{Image to Sequence}
%  the CNN-based encoder-T-decoder style transfer structure adopts a fixed pre-trained VGG to extract image content and style feature.
% However, the fixed pre-trained VGG includes pooling operation which will lead to the information leak.
% To prove that, in our model,
% Firstly, we show the stylziation results in \Cref{fig:ItoS}, from that we can conclude that the VGG projection layer can lead to style and content decay, and the results face the edge overflow problem (the first first row in \Cref{fig:ItoS}).
%\paragraph{Image to sequence.}

\inputfigure{fig_supp_ItoS}

\paragraph{Linear projection layer.}
As described in Section 1 of our main text, CNN-based style transfer structures may have issues of content leak after several rounds of the stylization process due to the details missing caused by locality and spatial invariance.
To show the impact of CNN structures, we replace the linear projection layer with a deep CNN projection layer to split the image into a sequence.
Fig.~\ref{fig:ItoS2} shows the stylization results after multiple rounds using different projection methods.
When increase the number of stylization rounds, the content structures generated by the CNN projection layer blur out, while the content structures generated by the linear projection layer are still distinct.

\vspace{-4pt}
\paragraph{Progressive generation.}
Thanks to the ability to capture long-range dependencies, transformer can be used to generate image in a progressive fashion without content leak.
% This progressive process restores the natural painting steps as far as possible.
We use three layers of transformer encoder-decoder to simulate the process of art creation from coarse to fine.
As depicted in Fig.~\ref{fig:progressive}, after remove the progressive layers and only use a single transformer layer, the results lose more structure details and the rendered style patterns become less similar to the reference style image (the square strokes in the sky).

In Table~\ref{tab:loss1}, we compute the content loss and style loss defined in Equations (9) and (10) of our main text. From this table we can see that our progressive generation scheme can increase both the content consistency and the style fidelity.
%the content maintaining and style transferring abilities are both degraded.
%
\inputfigure{fig_supp_progressive}

\vspace{-4pt}
\paragraph{Training weights.}
The loss weights $\lambda_{c}$, $\lambda_{s}$, $\lambda_{id1}$, and $\lambda_{id2}$ are adopted to eliminate the impact of magnitude differences.
We change $\lambda_{s}$ from $10$ to $5$ to evaluate the impact of style weight value.
Fig.~\ref{fig:weight} shows that reducing style weight leads to less obvious stylized patterns in the final output but the overall results still look reasonable.

\inputtable{tab_supp_progressive}
\inputfigure{fig_supp_weights}
\inputfigure{fig_vit}

\vspace{-4pt}
\paragraph{Loss function.}
StyTr$^2$ is trained using a pretrained VGG model which is not free of CNNs completely.
We try to use a pretrained VIT~\cite{dosovitskiy2021vit} model to extract features and construct content and style loss.
We use the VIT-based loss to train a new model and show some results in Fig.~\ref{fig:vit}.

The content structures are well preserved but very few style patterns are transferred.
Due to the global modeling ability of transformer, local texture patterns are difficult to be discovered.
We leverage the pretrained VGG model to integrate some priors of local texture patterns.
Therefore, our results can preserve both complete content structures and vivid style patterns.

% \subsection{Limitations}
% When we input a large content image of face and an abstract style image, the generated results can be rendered with plenty of style patterns (e.g., sharp edges in \Cref{fig:bad_case}) which may not be visually pleasant.
% The reason for the above phenomenon is that we do not consider whether the input style is suitable for the content image.
% In the future, we plan to take the semantic information of content and style into consideration to generate better stylization results.
% \inputfigure{fig_limitation}

% \paragraph{The influence of long-range information.}
% The input image is split into a patch sequence by a backbone CNN layer.
% This sequence contains image local information.
% The role of transformer encoder is to extract long-range dependencies synergistic with local features.
% In this section, we explore the influence of long-range information extracted by the transformation encoder.
% We remove the transformation encoder for comparison.
% From \Cref{fig:transformer_encoder}, without transformation encoder, the model can not be convergent. Although the network can learn some localized information(e.g., the rough outline of the character), the overall semantic structures are damaged.



% \inputfigure{transformer_encoder}
\section{Robustness Analysis}

Solving the content leak problem proves from the side that our method has a strong ability of transferring the content information of $I_c$ into $I_{cs}$.
However, we argue that robust content feature extraction and representation are the foundation of image style transfer.
From Figure 5 of our main text we can see that $I_{cs}^{1}$ and $I_{cs}^{20}$ are almost the same by ArtFlow, which indicates that when the input contents are totally different ($I_{c}$ for $I_{cs}^{1}$ while $I_{cs}^{19}$ for $I_{cs}^{20}$), the generated results could be the same.
Such phenomenon inspires us to further analyze the ability of content feature extraction for ArtFlow.
To verify the robustness of different methods, we add small perturbation into the multi-round stylization process, that is:
\begin{equation}
\begin{split}
I_{cs}^{i} = G_i( G\dots(G_1(I_c+ \Delta, I_s), \dots)+\Delta , I_s),
 \end{split}
\end{equation}
where $\Delta \sim \mathcal{N}(0, \sigma^2 I)$ is a small perturbation following a standard Gaussion distribution.
We show the stylization results after the \engordnumber{1}, \engordnumber{2}, \engordnumber{5}, and \engordnumber{10} rounds in Fig.~\ref{fig:noise}.
The small perturbation brings little impact to our results, but leads to significant content drop-out problem for ArtFlow.
Such results prove that although ArtFlow is good at maintaining the content information, the content representation mechanism is not robust to small perturbation.
Moreover, Fig.~\ref{fig:noise} demonstrates that flow-based model suffers from the problem of poor representation learning.
% In Fig.~\ref{fig:noise}, we compare the model robustness of our method with ArtFlow.
% As shown in the \engordnumber{4} and \engordnumber{7} columns in Fig.~\ref{fig:noise}, the perturbation $\Delta \sim \mathcal{N}(0, \sigma^2 I)$ is add to the stylized images, and that is small that can not be observed by human eyes.
% The small perturbation bring little impact in our results, but bring in huge content drop-out problem for ArtFlow.
\inputfigure{fig_supp_noise}

\inputfigure{fig_supp_big}

\section{More Qualitative Comparison Results}
In Fig.~\ref{fig:big}, we show our results in the resolution of $768 \times 768$.
In the generated results, the outline of content structures is clear (e.g., the mountains and buildings in the first and second rows, the animals in the third and fourth rows), and details of style patterns are well preserved (the pencil strokes in the second and fourth rows).
In Figs.~\ref{fig:content_leak_s}, \ref{fig:sup1}, \ref{fig:sup2}, \ref{fig:sup3} and \ref{fig:sup4}, we show more results to compare our method with AdaIN~\cite{Huang:2017:Arbitrary}, AAMS~\cite{yao:2019:attention}, DFP~\cite{wang:2020:diversified}, MCC~\cite{deng:2021:arbitrary}, and ArtFlow~\cite{an:2021:artflow}.

\inputfigure{fig_content_leak_s}
\inputfigure{fig_sup1}
\inputfigure{fig_sup2}
\inputfigure{fig_sup3}
\inputfigure{fig_sup4}

% \section{Comparisons with more contrast methods}
% In this section, we compare our model with Avatar~\cite{sheng:2018:avatar}, SANet~\cite{park:2019:arbitrary}, MAST~\cite{deng:2020:arbitrary}, StyleFormer~\cite{wu:2021:styleformer} and IEST~\cite{chen:2021:iest} in Figure~\ref{fig:sup_compare} and Figure~\ref{fig:sup_bias}.

% Firstly, we compare the first round stylization results.
% The decorator module in Avatar~\cite{sheng:2018:avatar} seriously damages the content structure information in the stylized results.
% SANet~\citep{park:2019:arbitrary}, MAST~\citep{deng:2020:arbitrary} and StyleFormer~\citep{wu:2021:styleformer} all use the self-attention mechanism, considering the correlation between style and content, but still facing the problems of insufficient style pattern and damaged content structure in the stylization results.
% Although IEST~\citep{chen:2021:iest} introduces contrastive loss to generate relatively realistic texture, the overall style of the results are quite different from that of the referenced style images.
% Secondly, with the increase of the stylization rounds, the content structures generated by CNN-based methods tend to be blurry, while the content structures generated by our method are still distinct.
%\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
%\centering
%\includegraphics[width= \linewidth]{image/figs_vits/sup_compare.pdf}
%\caption{Comparisons of style transfer results using different methods. 
%}
% \vspace{-4mm}
%\label{fig:sup_compare}
%\end{figure*}

%\begin{figure*}%[t]
%\setlength{\abovecaptionskip}{2mm}
%\centering
%\includegraphics[width= \linewidth]{image/figs_vits/sup_bias.pdf}
%\caption{A comparison of the Content Leak phenomenon.
%}
% \vspace{-4mm}
%\label{fig:sup_bias}
%\end{figure*}

\section{Dataset License}
Our model is trained on MS-COCO~\cite{lin:2014:coco} and WikiArt~\cite{phillips:2011:wiki}.
According to license of {MS-COCO}\footnote{\url{https://creativecommons.org/licenses/by-nc-sa/2.0/}}, we are allowed to copy and redistribute the material in any medium or format, remix, transform, and build upon the material.
{WikiArt}\footnote{\url{https://www.wikiart.org/en/terms-of-use}} can be used as historically significant artworks.

\section{Broader Impacts}
Compared to the CNN-based models, the transformer-based model brings some breakthroughs to style transfer.
StyTr$^2$ uses the strong representation and relationship modeling ability of the transformer to avoid the image details missing and to improve the stylization effect.
There can be some enlightenment for other vision tasks to use the specialties of transformers to enhance performance.
Moreover, this work is proposed for promising painting creation using referenced content and style images.
Although the application of this technique cannot threaten personal safety, deep fake could be used by crooks.


==> Sections/sup_section.tex <==
 
\section{Qualitative Comparison with StyleDiff}
% Figure \ref{fig:diff} showcases a comprehensive comparative study with StyleDiff~\cite{li2023stylediffusion}. In the first and second columns, we observe that when employing images from the CelebA-HQ~\cite{liu2015faceattributes} dataset as content images, the stylized output exhibits a resemblance to the input face but fails to capture the intricate style patterns. On the other hand, in the third and fourth columns, when extending the analysis beyond the confines of the pre-trained dataset, the stylized output becomes perplexing and loses its intended style representation.
Figure \ref{fig:diff} presents a detailed comparative analysis conducted in conjunction with StyleDiff~\cite{li2023stylediffusion} to assess the performance of different methods. By utilizing images from the CelebA-HQ~\cite{liu2015faceattributes} dataset as content images, we observe in the first and second columns that the stylized output demonstrates a certain degree of resemblance to the input face. However, it falls short in capturing the intricate style patterns effectively. 

Expanding our investigation beyond the limitations of the pre-trained dataset, as depicted in the third and fourth columns, we encounter a perplexing scenario where the stylized output loses its intended style representation. This outcome highlights the challenges associated with maintaining the desired style when confronted with unfamiliar or out-of-domain content.

\section{Visualization of Content Style Correlation}
% Figure \ref{fig:cross_attention_images} presents the visualization of the content-style correlation outcomes, i.e., the outputs of Softmax($Q_cK_s$). It is shown that a stable diffusion model can naturally leverage the correlation between the content query and style key that has similar semantic information, without retraining. Since the content and style images are already aligned with cross-attention, it inspires us to propose the dual path network to transfer the style to the content images with the improved attention mechanism. 
% In Figure \ref{fig:cross_attention_images}, we observe the visual representation of the outcomes of the content-style correlation analysis, specifically the results obtained from Softmax($Q_cK_s$). The visualization demonstrates that a well-trained diffusion model~\cite{ddim_paper} can effectively exploit the correlation between the content query and style key, which possess similar semantic information, without requiring retraining. This observation, where the content and style images are already aligned through cross-attention, serves as inspiration for our proposed dual-path network. This network incorporates an enhanced attention mechanism to facilitate the transfer of style to the content images.
Figure \ref{fig:cross_attention_images} showcases the visual depiction of the results obtained from the content-style correlation analysis, focusing specifically on the outcomes derived from Softmax($Q_cK_s$). The visualization provides evidence that a well-trained diffusion model~\cite{ddim_paper} can effectively leverage the correlation between the content query and style key, which possess similar semantic information, without necessitating retraining. This observation, where the alignment of content and style images is achieved through cross-attention, serves as a source of inspiration for our proposed dual-path network. This network incorporates an enhanced attention mechanism to facilitate the transfer of style to the content images, thereby improving the overall style transfer performance. 

Our method exploits the inherent relationship between content and style by incorporating a more advanced attention mechanism, which enables the network to selectively focus on relevant style information and effectively transfer it to the content images. By leveraging the insights gained from the content-style correlation analysis, we anticipate that our proposed approach will lead to enhanced style transfer results, surpassing the limitations of existing methods.

\inputfigure{fig_diff.tex}

\section{Proof of Equation (14)}
To enhance the clarity of the derivation process, the proof commences on a fresh page.
\onecolumn
\begin{proof}
% \begin{strip}
\begin{align}
    \hat{f}_c&=\frac{1}{2}\cdot\text{Attn}(Q_c,K_s,V_s)+\frac{1}{2}\cdot\text{Attn}(Q_c,K_c,V_c)=\frac{1}{2}\cdot\text{Softmax}(\frac{Q_cK_s^T}{\sqrt{d}})V_s+\frac{1}{2}\cdot\text{Softmax}(\frac{Q_cK_c^T}{\sqrt{d}})V_c
\end{align}
Note that the matrix $\hat{f}_c$ can be expressed as a combination of individual elements. To simplify the derivation process, we focus on each element $\hat{f}_c^{i,j}$
\begin{align}
\hat{f}_c^{i,j}=\frac{1}{2}\cdot\text{Softmax}(\frac{[Q_{c}]_{i,\cdot}K_s^T}{\sqrt{d}})[V_{s}]_{\cdot, j}+
\frac{1}{2}\cdot\text{Softmax}(\frac{[Q_{c}]_{i, \cdot}K_c^T}{\sqrt{d}})[V_{c}]_{\cdot, j}
\end{align}
where $[Q]_{i,\cdot}\in\mathbb{R}^{1\times N}$ corresponds to the $i$-th row in matrix $Q$ and $[V]_{\cdot,j}\in\mathbb{R}^{N\times 1}$ indicates the $j$-th column in matrix $V$. To facilitate the derivation, we introduce two intermediate variables:
\begin{align}
x^{cs}=\frac{1}{\sqrt{d}}\cdot[Q_{c}]_{i,\cdot}K_s^T, \qquad x^{cc}=\frac{1}{\sqrt{d}}\cdot[Q_{c}]_{i,\cdot}K_c^T
\end{align}
where $x^{cs},x^{cc}\in\mathbb{R}^{1\times N}$. Expanding the Softmax formulation, we express $\hat{f}_c^{i,j}$ as a weighted sum over $N$ elements:
\begin{align}
\hat{f}_c^{i,j}&=\frac{1}{2}\cdot\sum_n^N\frac{\exp(x^{cs}_n)}{\sum_{m}^N\exp(x^{cs}_m)}[V_{s}]_{k, j}+
\frac{1}{2}\cdot\sum_n^N\frac{\exp(x^{cc}_n)}{\sum_{m}^N\exp(x^{cc}_m)}[V_{c}]_{k, j}\\
&=\frac{1}{2}\cdot\sum_n^N\frac{\exp(x^{cs}_n)}{\sum_{m}^N\exp(x^{cs}_m)}[V_{s}]_{k, j}+\frac{\exp(x^{cc}_n)}{\sum_{m}^N\exp(x^{cc}_m)}[V_{c}]_{k, j}\\
&=\frac{1}{2}\cdot\sum_n^N\frac{\exp(x^{cs}_n)[V_{s}]_{k, j}\sum_{m}^N\exp(x^{cc}_m)}{\sum_{m}^N\exp(x^{cc}_m)\sum_{m}^N\exp(x^{cs}_m)}+
    \frac{\exp(x^{cc}_n)[V_{c}]_{k, j}\sum_{m}^N\exp(x^{cs}_m)}{\sum_{m}^N\exp(x^{cc}_m)\sum_{m}^N\exp(x^{cs}_m)}\\
&=\sum_n^N\frac{\exp(x^{cs}_n)[V_{s}]_{k, j}\sum_{m}^N\exp(x^{cc}_m)+\exp(x^{cc}_n)[V_{c}]_{k, j}\sum_{m}^N\exp(x^{cs}_m)}{2\sum_{m}^N\exp(x^{cc}_m)\sum_{m}^N\exp(x^{cs}_m)}\\
&=\sum_n^N\frac{\exp(x^{cs}_n)[V_{s}]_{k, j}\sum_{m}^N\exp(x^{cc}_m)+\exp(x^{cc}_n)[V_{c}]_{k, j}\sum_{m}^N\exp(x^{cs}_m)}{\sum_{m}^N\exp(x^{cc}_m)\sum_{m}^N\exp(x^{cs}_m)+\sum_{m}^N\exp(x^{cc}_m)\sum_{m}^N\exp(x^{cs}_m)}\\
&=\sum_n^N\frac{\exp(x^{cs}_n)[V_{s}]_{k, j}\frac{\sum_{m}^N\exp(x^{cc}_m)}{\sum_{m}^N\exp(x^{cs}_m)}+\exp(x^{cc}_n)[V_{c}]_{k, j}}{\sum_{m}^N\exp(x^{cs}_m)\frac{\sum_{m}^N\exp(x^{cc}_m)}{\sum_{m}^N\exp(x^{cs}_m)}+\sum_{m}^N\exp(x^{cc}_m)}
\end{align}
Upon rewriting the equation $\ln\frac{\sum_{m}^N\exp(x^{cc}_m)}{\sum_{m}^N\exp(x^{cs}_m)}=C$, we obtain the resulting expression
\begin{equation}
\hat{f}_c^{i,j}=\sum_n^N\frac{\exp(x^{cs}_n+C)[V_{s}]_{k, j}+\exp(x^{cc}_n)[V_{c}]_{k, j}}{\sum_{m}^N\exp(x^{cs}_m+C)+\sum_{m}^N\exp(x^{cc}_m)}=\text{Softmax}([x^{cs}+C, x^{cc}])*\left[
   \begin{matrix}
       [V_s]_{\cdot,j}\\
       [V_c]_{\cdot,j}
\end{matrix}\right]
\end{equation}
By substituting the derived expression for $\hat{f}_c^{i,j}$ into the matrix form, we obtain the formulation presented in Equation (8).
\end{proof}

\twocolumn

\begin{figure}[th!]
\begin{center}
\begin{minipage}[t]{.09\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{./images/limitation/28_content_62_style_source.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/28_content_62_style_source.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/49_content_62_style_source.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/49_content_62_style_source.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/51_content_51_style_source.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/51_content_51_style_source.png}
  \caption*{(a) Content}
\end{minipage}
\begin{minipage}[t]{.09\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{./images/limitation/49_content_28_style_style.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/Landscape02_c_Boat_s_source_33_style_style.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/49_content_28_style_style.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/Landscape02_c_Boat_s_source_33_style_style.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/49_content_28_style_style.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/Landscape02_c_Boat_s_source_33_style_style.png}
  \caption*{(b) Style I}
\end{minipage}
\begin{minipage}[t]{.09\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{./images/limitation/28_content_28_style_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/28_content_33_style_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/49_content_28_style_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/49_content_33_style_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/51_content_28_style_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/51_content_33_style_reconstructed.png}
  \caption*{(c) Result I}
\end{minipage}
\begin{minipage}[t]{.09\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{./images/limitation/49_content_62_style_style.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/Landscape02_c_Boat_s_source_51_style_style.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/49_content_62_style_style.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/Landscape02_c_Boat_s_source_51_style_style.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/49_content_62_style_style.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/Landscape02_c_Boat_s_source_51_style_style.png}
  \caption*{(d) Style II}
\end{minipage}
\begin{minipage}[t]{.09\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{./images/limitation/28_content_62_style_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/28_content_51_style_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/49_content_62_style_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/49_content_51_style_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/51_content_62_style_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/limitation/51_content_51_style_reconstructed.png}
  \caption*{(e) Result II}
\end{minipage}
\caption{We present a visual representation of the style transfer outcomes achieved by applying landscape image styles to both landscape and portrait images, as well as vice versa. While our method demonstrates promising results in the context of style transfer within the same domain (as evidenced by the 1st, 3rd, and last rows), there is room for improvement when transferring portrait styles to landscape images, as illustrated by the 2nd and 4th rows.}
\label{fig:limitation}
\end{center}
\end{figure}

%%%%%%% Cross-Attention Visualization %%%%%%%%%%%%
\begin{figure*}[t!]
 \centering
 % Line 1
 \includegraphics[width=0.11\textwidth]{images/cross_attention/portrait_content.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_10_22__content.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_10_28__content.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_16_14__content.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_18_6__content.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_22_attention_cs_18_18__content.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_22_attention_cs_22_4__content.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_22_attention_cs_26_16__content.png}
 % Line 2
 \includegraphics[width=0.11\textwidth]{images/cross_attention/portrait_style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_10_22__style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_10_28__style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_16_14__style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_18_6__style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_22_attention_cs_18_18__style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_22_attention_cs_22_4__style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_22_attention_cs_26_16__style.png}
  % Line 3
 \includegraphics[width=0.11\textwidth]{images/cross_attention/landscape_content.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_2_10__content.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_8_12__content.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_14_2__content.png}
 \includegraphics[width=0.11\textwidth]
 {images/cross_attention/5_20_attention_cs_18_7__content.png}
 \includegraphics[width=0.11\textwidth]
 {images/cross_attention/5_20_attention_cs_16_30__content.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_28_26__content.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_32_26__content.png}
 % Line 4
 \includegraphics[width=0.11\textwidth]{images/cross_attention/landscape_style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_2_10__style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_8_12__style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_14_2__style.png}
 \includegraphics[width=0.11\textwidth]
 {images/cross_attention/5_20_attention_cs_18_7__style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_16_30__style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_28_26__style.png}
 \includegraphics[width=0.11\textwidth]{images/cross_attention/5_20_attention_cs_32_26__style.png}
 \caption{Visualization of cross-attention results. The first and third rows pertain to the content images, whereas the second and last rows pertain to the style images. The highlighted blocks in the content images denote the content queries, while the highlighted regions in the style images correspond to the relevant regions of the corresponding content query blocks, as determined via the Softmax function in cross-attention with high values.}
 \label{fig:cross_attention_images}
\end{figure*}



\begin{figure*}[th]
\begin{center}
\begin{minipage}[t]{.13\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{./images/lambda/117531700228184_.pic_117541700228192_.pic_source.png}
  \includegraphics[width=1.\linewidth]{./images/lambda/117551700228198_.pic_117561700228206_.pic_source.png}
  \caption*{(a) Content}
\end{minipage}
\begin{minipage}[t]{.13\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{./images/lambda/117531700228184_.pic_117541700228192_.pic_style.png}
  \includegraphics[width=1.\linewidth]{./images/lambda/117551700228198_.pic_117561700228206_.pic_style.png}
  \caption*{(b) Style}
\end{minipage}
\begin{minipage}[t]{.13\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{./images/lambda/0.1/117531700228184_.pic_117541700228192_.pic_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/lambda/0.1/117551700228198_.pic_117561700228206_.pic_reconstructed.png}
  \caption*{(c) $\lambda=0.1$}
\end{minipage}
\begin{minipage}[t]{.13\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{./images/lambda/0.3/117531700228184_.pic_117541700228192_.pic_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/lambda/0.3/117551700228198_.pic_117561700228206_.pic_reconstructed.png}
  \caption*{(d) $\lambda=0.3$}
\end{minipage}
\begin{minipage}[t]{.13\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{./images/lambda/0.5/117531700228184_.pic_117541700228192_.pic_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/lambda/0.5/117551700228198_.pic_117561700228206_.pic_reconstructed.png}
  \caption*{(e) $\lambda=0.5$}
\end{minipage}
\begin{minipage}[t]{.13\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{./images/lambda/0.7/117531700228184_.pic_117541700228192_.pic_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/lambda/0.7/117551700228198_.pic_117561700228206_.pic_reconstructed.png}
  \caption*{(f) $\lambda=0.7$}
\end{minipage}
\begin{minipage}[t]{.13\textwidth}
  \centering
  \includegraphics[width=1.\linewidth]{./images/lambda/0.9/117531700228184_.pic_117541700228192_.pic_reconstructed.png}
  \includegraphics[width=1.\linewidth]{./images/lambda/0.9/117551700228198_.pic_117561700228206_.pic_reconstructed.png}
  \caption*{(g) $\lambda=0.9$}
\end{minipage}
\caption{We investigate the impact of the $\lambda$ parameter in Equation (8), specifically in the context of Simple Addition. We present a visual representation of the outcomes obtained when the style and content images exhibit a lack of correlation (i.e., a challenging sample) in the first row, and when the content and style images are similar (an easier sample) in the second row. Notably, we observe that the second row consistently yields favorable visualization results when $\lambda$ is set to 0.9. However, the first row fails to achieve a satisfactory balance between the content and style. For instance, when $\lambda$ is low, the content is well preserved at the expense of losing the style, and vice versa.}
\label{fig:lambda_simple_addition}
\end{center}
\end{figure*}

\section{Impact of $\lambda$ in Equation (8)}
% In contrast to the robustness of the $\lambda$ in Attention Rearrangement, the $\lambda$ is hard to make a balance between the style and content feature in Equation (8). We illustrate the results in Figure \ref{fig:lambda_simple_addition} with a relatively hard style transfer image pair and an easy sample to explain the problem.
Unlike the resilient nature of the $\lambda$ parameter in Attention Reweighting, achieving a suitable balance between the style and content features in Equation (8) proves to be challenging. To elucidate this issue, we present the outcomes in Figure \ref{fig:lambda_simple_addition}, employing a pair of style transfer images that exhibit varying levels of difficulty in style transfer.

\section{Quantitative Analysis}
For quantitative comparison with state-of-the-art methods, we employ content loss and style loss as evaluation metrics to assess the preservation of content and rendering of style, respectively.
% To compare our method with the State-of-the-art methods quantitatively, we use content loss and style loss to evaluate the content preservation and style rendering ability.
Content loss and style loss are commonly adopted in style transfer tasks, defined as:
\begin{equation}
\begin{split}
\contentloss = \frac{1}{\layernumber}\sum_{ i=0 }^{\layernumber} \lVert \phi_i(\outputimage) - \phi_i(\inputcontent)  \lVert_2,
\end{split}
\label{fun:contentloss}
\end{equation}
%
where $\phi_i(\cdot)$ denotes features extracted from the $i$-th layer in a pre-trained VGG19 and $\layernumber$ is the number of layers. The style perceptual loss $\styleloss$ is defined as
\begin{equation}
\begin{split}
\styleloss = \frac{1}{\layernumber}\sum_{ i=0 }^{\layernumber}& \lVert \mu( \phi_i(\outputimage)) - \mu (\phi_i(I_{s})) \lVert_2 \\
&+ \lVert \sigma( \phi_i(\outputimage)) - \sigma (\phi_i(I_{s})) \lVert_2,
\end{split}
\label{fun:styleloss}
\end{equation}
where $\mu(\cdot)$ and $\sigma (\cdot)$ denote the mean and variance of extracted features, respectively. The content loss is computed using the features extracted from the $5$-th layer, while the style loss is calculated using the features from the $1$-st to $5$-th layers.

The outcomes of the comparative analysis are presented in Table~\ref{tab:quancomps}. Our proposed method achieves the lowest style loss, indicating its superior ability to render style. On the other hand, StyTr$^2$~\cite{Deng:2022:CVPR} achieves the lowest content loss, highlighting its effectiveness in preserving content. Notably, our method demonstrates relatively low values for both content and style loss, suggesting a favorable balance between content preservation and style rendering.

We also performed further quantitative analysis for the ablation study, detailed in Table~~\ref{tab:abl}, which supports the findings discussed in the ablation study. 

\begin{table*}[!t]

\renewcommand\arraystretch{0.9}
    \centering
    \caption{Quantitative results for ablation study}
    \vspace{-10pt}
	\begin{minipage}{0.3\linewidth}
		\centering
        \begin{tabular}{ccc}
    \toprule
    &$\contentloss$ &$\styleloss$ \\
    \midrule
    ours & 1.61  & 3.70     \\
    step 0-10     &  2.70&    3.56   \\
    step 10-20     &  1.17     &  4.56

 \\
    step 20-30     &  0.11
       & 5.03  \\
    step 5-20     &   1.37
      &  4.13 \\
    
    \bottomrule
\end{tabular}
        % \caption{The crane}
        %\label{table:NormalSafe}
	\end{minipage}
	%\qquad
	\hfill
	\begin{minipage}{0.3\linewidth}
		\centering
        \begin{tabular}{ccc}
    \toprule
    &$\contentloss$ &$\styleloss$ \\
    \midrule
    step 15-30     &  1.25
       &  4.53 \\
    Simple Add &  1.86
  &   4.64       \\
    Naïve Set   & 1.92
 &      3.96     \\
    layer 0-5     & 2.16
 &   4.81
    \\
    layer 5-10     &   0.96
      &  6.17
 \\
    
    \bottomrule
\end{tabular}
        % \caption{The crane}
        \label{table:NormalSafe}
	    \end{minipage}
\hfill
    \begin{minipage}{0.3\linewidth}
		\centering
        \begin{tabular}{ccc}
    \toprule
    &$\contentloss$ &$\styleloss$ \\
    \midrule
    layer 0-15     &    2.46
     &  4.04
 \\
    $\lambda$ = 1.0    &    1.04
     &  4.80 \\
    $\lambda$ = 1.1     &    1.56
     &  4.22\\
    $\lambda$ = 1.3     &  2.08
       & 3.47
  \\
    $\lambda$ = 1.4     &    2.18
     &  3.30 \\
    \bottomrule
\end{tabular}
        % \caption{The crane}
        %\label{table:NormalSafe}
	\end{minipage}
	%\qquad
	\hfill

\label{tab:abl}
\end{table*}


\begin{table*}%[!h]
\small
%\setlength\tabcolsep{2.5pt}
\centering
%\begin{adjustbox}{width=\textwidth,center}
\caption{Quantitative comparisons. To evaluate the preservation of input content and style, we calculate the average values of content and style loss for the results obtained through various methods. The most favorable outcomes are highlighted in \textbf{bold}.}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccccccccc}
\toprule
%\resizebox{\textwidth}
%  & Ours & AdaAttN &ArtFlow & MCC &  AAMS & AdaIN \\
  &ours& VCT~\cite{cheng:2023:ict}& StyleDiff~\cite{jeong:2023:hspace}&InST~\cite{zhang:2023:inversion}&QuanArt~\cite{huang2023quantart}&CAST~\cite{zhang:2022:domain}&StyTr$^2$~\cite{Deng:2022:CVPR} & IEST~\cite{chen:2021:iest} &AdaAttN~\cite{liu:2021:adaattn}&  ArtFlow~\cite{an:2021:artflow}  \\
\midrule
$\contentloss$ &  1.61&1.73 &3.55 &   2.85 & 1.71 & 1.66 &  \textbf{1.59} &  1.82&1.89&1.93 \\
\midrule
$\styleloss$  & \textbf{3.70} &3.98&  4.01 &4.70 & 5.50& 4.18&3.79   & 3.86&3.78&4.32 \\
\bottomrule
\end{tabular}
}
% \vspace{-10pt}
\label{tab:quancomps}
%\vspace{-5pt}
\end{table*}

\section{Visual Comparison with SOTA}
In order to provide further evidence of the effectiveness of our proposed method, we present additional results in Figures~\ref{fig:sup1} and \ref{fig:sup2}. These figures demonstrate the performance of our method across a range of image genres, including portraits and landscapes, as well as concrete and abstract styles. The results consistently indicate the strong performance and versatility of our method in handling various image styles.

\section{Limitations}
Like a coin with two sides, the attention-based zero-shot style transfer method presents a nuanced evaluation with both positive and negative aspects. The favorable outcomes of this approach benefit the utilization of a pre-trained stable diffusion model, which is also widely acknowledged to yield varying quality results based on the input data. Through our rigorous experimentation, we discovered a potential limitation of our method when transferring style information from portraits to landscape images. To facilitate a comprehensive understanding, we have included a visual comparison of the results in Figure \ref{fig:limitation}.



\inputfigure{fig_sup1.tex}
\inputfigure{fig_sup2.tex}

==> Tables/tab_supp_progressive.tex <==
\begin{table}%[!h]
\small
\setlength\tabcolsep{2.5pt}
\centering
\begin{tabular}{c|c|c}
\toprule
&Single-layer &Ours (multi-layer)  \\
\midrule
$\contentloss$ $\downarrow$ & 1.94& \textbf{1.91} \\
$\styleloss$ $\downarrow$ & 2.38 & \textbf{1.47}  \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\caption{Quantitative evaluation of progressive generation.}
\label{tab:loss1}
\end{table}


==> Tables/tab_timing_comparison.tex <==
\begin{table*}%[!h]
%\small
%\setlength\tabcolsep{2.5pt}
\centering
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{c|ccccccccccc}
\toprule
Resolution & Ours & StyleFormer&IEST&AdaAttN&ArtFlow & MCC &MAST&  AAMS & SANet&Avatar&AdaIN \\
\midrule
256 $\times$ 256&0.116 & 0.013&0.065& 0.104 & 0.142 & 0.013 &0.030& 2.074 & 0.015&0.260&0.007 \\
\midrule
512 $\times$ 512 & 0.661& 0.026& 0.092& 0.213 & 0.418 & 0.015  & 0.096&2.173 &0.019& 0.470&0.008 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-5pt}
\caption{Average inference time (in seconds) of different methods at two output resolutions.}
\label{tab:time}
\vspace{-7pt}
\end{table*}


==> Tables/tab_user_study.tex <==
% \begin{table}
%     \centering
%     \begin{subtable}[t]{\linewidth}
%         \begin{tabular}{c|ccccc}
%             \toprule
%             &ArtFlow&MCC&DFP& AAMS& AdaIN \\
%             \midrule
%             % Num. & 783&820&827&809&734 \\
%             votes(\%) &25.7&25.5&22.6&18.2& 23.5\\
%             % Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
%             \bottomrule
%         \end{tabular}
%         \caption{Overall}
%     \end{subtable}
%     \begin{subtable}[t]{\linewidth}
%     \begin{tabular}{c|ccccc}
%         % \begin{tabular}{m{0.6cm}<{\centering}|m{0.8cm}<{\centering}m{0.5cm}<{\centering}m{0.4cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
%             \toprule
%             &ArtFlow&MCC&DFP& AAMS& AdaIN \\
%             \midrule
%             % Num. & 783&820&827&809&734 \\
%             votes(\%) &28.3&20.6&9.2&19.4& 31.7\\
%             % Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
%             \bottomrule
%         \end{tabular}
%         \caption{Content}
%     \end{subtable}
%     \begin{subtable}[t]{\linewidth}
%         % \begin{tabular}{m{0.7cm}<{\centering}|m{0.7cm}<{\centering}m{0.5cm}<{\centering}m{0.5cm}<{\centering}m{0.6cm}<{\centering}m{0.6cm}<{\centering}}
%         \begin{tabular}{c|ccccc}
%             \toprule
%             &ArtFlow&MCC&DFP& AAMS& AdaIN \\
%             \midrule
%             % Num. & 783&820&827&809&734 \\
%             votes(\%) &16.7&27.8&28.2&14.8& 13.5\\
%             % Vote rate$\uparrow$ &\textbf{0.398}&0.138&0.136&0.116& 0.089& 0.123 \\
%             \bottomrule
%         \end{tabular}
%         \caption{Style}
%     \end{subtable}
%     \caption{User study results.}
%     \label{tab:user_study}
% \end{table}
\begin{table}
\centering
\begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{l|ccccc}
    \toprule
    &AdaAttN&ArtFlow & MCC  & AAMS & AdaIN \\
    \midrule
    Overall & 44.8\%&25.7\% & 25.5\%  & 18.2\% & 23.5\% \\
    \midrule
    Content & 45.7\%&28.3\% & 20.6\% & 19.4\%&  31.7\% \\
    \midrule
    Style & 23.6\%&16.7\% & 27.8\% & 14.8\% & 13.5\% \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\vspace{-5pt}
\caption{User study results. Each number represents the percentage of votes that the corresponding method is preferred to ours, using the criteria of overall quality, preservation of content and style, respectively.}
\label{tab:user_study}
\vspace{-10pt}
\end{table}

